Batch Normalization Embeddings for Deep Domain Generalization

Domain generalization aims at training machine learning models to perform robustly across different and unseen domains. Several recent methods use multiple datasets to train models to extract domain-invariant features, hoping to generalize to unseen domains. Instead, first we explicitly train domain-dependant representations by using ad-hoc batch normalization layers to collect independent domain's statistics. Then, we propose to use these statistics to map domains in a shared latent space, where membership to a domain can be measured by means of a distance function. At test time, we project samples from an unknown domain into the same space and infer properties of their domain as a linear combination of the known ones. We apply the same mapping strategy at training and test time, learning both a latent representation and a powerful but lightweight ensemble model. We show a significant increase in classification accuracy over current state-of-the-art techniques on popular domain generalization benchmarks: PACS, Office-31 and Office-Caltech.

==> figures/gaussians.tex <==
%
%% BEGIN FIGURE GAUSSIANS
\begin{figure*}
\centering
%\scalebox{0.85}{
\subfloat[Creation of domain representations.]{{\includegraphics[trim=0cm 0cm 16cm 3.83cm, clip, width=0.31\linewidth,height=4.5cm]{img/blobs_0.pdf}}}
\quad
\subfloat[Projection of a sample from an unknown domain.]{{\includegraphics[trim=0cm 0cm 16cm 3.83cm, clip, width=0.31\linewidth,height=4.5cm]{img/blobs_1.pdf}}}
\quad
\subfloat[Localization with respect to known domains.]{{\includegraphics[trim=0cm 0cm 16cm 3.83cm, clip, width=0.31\linewidth,height=4.5cm]{img/blobs_2.pdf}}}
%}
\caption{We propose to: (a) learn domain specific models and map training domains (in red) in a latent space via population statistics of the BN layers, (b) project a sample from an unknown domain to the same space via its instance statistics (in green), and (c) measure its distance from the known domains to approximate the unknown test distribution by a mixture of the domain models.}
\label{fig:gaussians}
\vspace{-0.5cm}
\end{figure*}

%% END FIGURE GAUSSIANS
%

==> figures/tsne.tex <==
%
%% BEGIN FIGURE t-SNE
\begin{figure} [h!]
\centering
\centering
\subfloat[Pacs]{{\includegraphics[trim=6cm 0cm 1cm 0cm, clip, width=0.45\linewidth]{img/pacs_tsne.pdf}}}
\qquad
\subfloat[Office-31]{{\includegraphics[trim=6cm 0cm 1cm 0cm, clip, width=0.45\linewidth]{img/office31_tsne.pdf}}}
\label{fig:tsne}
\caption{T-SNE}
\end{figure}
%% END FIGURE t-SNE
%

==> figures/tsne_layers.tex <==
% %
% %% BEGIN FIGURE t-SNE
% \begin{figure}
% \centering
% \centering
% \subfloat[BN Layer 1]{{\includegraphics[trim=0cm 0cm 16cm 5.5cm, clip, width=0.33\linewidth]{img/tsne_1.pdf}}}
% % \qquad
% \subfloat[BN Layer 2]{{\includegraphics[trim=0cm 0cm 16cm 5.5cm, clip, width=0.33\linewidth]{img/tsne_2.pdf}}}
% % \qquad
% \subfloat[BN Layer 3]{{\includegraphics[trim=0cm 0cm 16cm 5.5cm, clip, width=0.33\linewidth]{img/tsne_3.pdf}}}
% % \qquad
% \newline
% % \vspace{-0.5cm}
% \subfloat[BN Layer 4]{{\includegraphics[trim=0cm 0cm 16cm 5.5cm, clip, width=0.33\linewidth]{img/tsne_4.pdf}}}
% % \qquad
% \subfloat[BN Layer 5]{{\includegraphics[trim=0cm 0cm 16cm 5.5cm, clip, width=0.33\linewidth]{img/tsne_5.pdf}}}
% % \qquad
% \subfloat[Legend]{{\includegraphics[trim=0cm 0cm 20cm 9.5cm, clip, width=0.33\linewidth]{img/tsne_legend.pdf}}}
% \label{fig:tsne}
% \caption{T-SNE}
% \end{figure}
% %% END FIGURE t-SNE
% %

%
%% BEGIN FIGURE t-SNE
\begin{figure} [h!]
\centering
\centering
\subfloat[BN-1]{{\includegraphics[trim=0cm 0cm 16cm 5.5cm, clip, width=0.2\linewidth]{img/tsne_1.pdf}}}
\subfloat[BN-2]{{\includegraphics[trim=0cm 0cm 16cm 5.5cm, clip, width=0.2\linewidth]{img/tsne_2.pdf}}}
\subfloat[BN-3]{{\includegraphics[trim=0cm 0cm 16cm 5.5cm, clip, width=0.2\linewidth]{img/tsne_3.pdf}}}
\subfloat[BN-4]{{\includegraphics[trim=0cm 0cm 16cm 5.5cm, clip, width=0.2\linewidth]{img/tsne_4.pdf}}}
\subfloat[BN-5]{{\includegraphics[trim=0cm 0cm 16cm 5.5cm, clip, width=0.2\linewidth]{img/tsne_5.pdf}}}
\caption{T-SNEs of the distribution of samples from PACS~\cite{li2017deeper} at different depths in our modified AlexNet~\cite{simon2016imagenet} architecture. Each point represents the instance statistics of a sample at a certain level in the network. The model is trained on the domains \textit{Art Painting} (pink), \textit{Cartoon} (red), \textit{Photo} (blue); \textit{Sketch} (cyan) is left unseen. Population statistics for seen domains are shown as green dots.}
\label{fig:tsne_layers}
\end{figure}
%% END FIGURE t-SNE
%

==> tables/SOTA-PACS-Resnet-old.tex <==

%% BEGIN TABLE SOTA PACS RESNET
\setlength{\tabcolsep}{4pt}
\begin{table*}[t]
\begin{center}
\caption{State-of-the-art comparison on \pacs{} with \resnet{}. Methods with * do not use domain labels.}
\label{table:SOTA-PACS-Resnet}
%\scalebox{0.8}{
\begin{tabular}{c|c c c c|c c c}
\hline\noalign{\smallskip}
Method & Art & Cartoon & Photo & Sketch & \averageDeepAll{} & \averagePerfomance{} & $\Delta \%$ \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
CrossGrad -~\cite{shankar2018generalizing} & 78.7 & 73.3 & 94.0 & 65.1 & 79.1 & 77.8 & -1.64 \\ %-2.63\\
MetaReg -~\cite{balaji2018metareg} &  79.9 & 75.1 & 95.2 & 69.5 & 79.9 & 81.7 & +2.25 \\ %+2.25 \\
MLDG -~\cite{li2018learning} &  79.5 & 77.3 & 94.3 & 71.5 & 79.1 & 80.7 & +2.02 \\ %+2.02 \\
Epi-FCR -~\cite{li2019episodic} &  82.1 & 77.0 & 93.9 & 73.0 & 79.1 & 81.5 & +3.03 \\ %+3.03 \\
JiGen* -~\cite{carlucci2019domain} &  79.4 & 75.3 & \textbf{96.0} & 71.4 & 79.1 & 80.5 & +1.77 \\ %+1.77 \\
MASF -~\cite{dou2019domain} &  80.3 & 77.1 & 94.99 & 71.69 & 79.2 & 81.0 & +1.01 \\ %+1.01 \\
D-SAM - \cite{d2018domain} & 77.3 & 72.4 & 95.3 & 77.8 & 79.5 & 80.7 & +1.47 \\
MMLD* - \cite{matsuura2020domain} & 81.3 & 77.2 & 96.1 & 72.3 & 78.7 & 81.8 & +3.93 \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
DeepAll &  75.8 & 73 & 94.4 & 70.9 & - & 78.5 & - \\
\methodName{} (\textit{Ours}) &  78.8 & \textbf{78.9} & 94.8 & \textbf{79.7} & 78.5 & \textbf{83.1} & \textbf{+5.86} \\ %\textbf{+5.52} \\
\hline
\end{tabular}
%}
\end{center}
\end{table*}
%% END TABLE SOTA PACS RESNET
%
